Are Labels Required for Improving Adversarial Robustness?

Recent work has uncovered the interesting (and somewhat surprising) finding that training models to be invariant to adversarial perturbations requires substantially larger datasets than those required for standard classification. This result is a key hurdle in the deployment of robust machine learning models in many real world applications where labeled data is expensive. Our main insight is that unlabeled data can be a competitive alternative to labeled data for training adversarially robust models. Theoretically, we show that in a simple statistical setting, the sample complexity for learning an adversarially robust model from unlabeled data matches the fully supervised case up to constant factors. On standard datasets like CIFAR-10, a simple Unsupervised Adversarial Training (UAT) approach using unlabeled data improves robust accuracy by 21.7% over using 4K supervised examples alone, and captures over 95% of the improvement from the same number of labeled examples. Finally, we report an improvement of 4% over the previous state-of-the-art on CIFAR-10 against the strongest known attack by using additional unlabeled data from the uncurated 80 Million Tiny Images dataset. This demonstrates that our finding extends as well to the more realistic case where unlabeled data is also uncurated, therefore opening a new avenue for improving adversarial training.

==> gaussian.tex <==
\newpage
\appendix
\section{Proofs for Gaussian Model}

\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\I}{\ensuremath{\mathbb{I}}}
\newcommand{\Eop}{\ensuremath{\mathop{\mathbb{E}}}}
\newcommand{\prob}{\ensuremath{\mathbb{P}}}
\newcommand{\probop}{\ensuremath{\mathop{\mathbb{P}}}}
\newcommand{\vz}{\ensuremath{z}}
\newcommand{\vpz}{\ensuremath{z'}}
\newcommand{\vx}{\ensuremath{x}}
\newcommand{\yhi}{\ensuremath{\hat{y}_i}}
\newcommand{\vzbar}{\overline{\ensuremath{z}}}
\newcommand{\vpzbar}{\overline{\ensuremath{z'}}}
\newcommand{\vhzbar}{\overline{\ensuremath{\hat{z}}}}
\newcommand{\zbar}{\overline{\ensuremath{z}}}
\newcommand{\vg}{\ensuremath{g}}
\newcommand{\vgbar}{\overline{\ensuremath{g}}}
\newcommand{\vw}{\ensuremath{w}}
\newcommand{\vmu}{\ensuremath{\mu}}
\newcommand{\what}{\ensuremath{\hat{w}}}
\newcommand{\matI}{\ensuremath{I}}
\newcommand{\thetastar}{\ensuremath{\theta^\star}}
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
\newcommand{\normal}{\ensuremath{\mathcal{N}}}
\newcommand{\M}{\ensuremath{\mathcal{M}}}
\newcommand{\rademacher}{\ensuremath{\mathcal{R}}}
\newcommand{\distP}{\ensuremath{\mathcal{P}}}
\newcommand{\powerset}{\ensuremath{\mathscr{P}}}
\newcommand{\perturbB}{\ensuremath{\mathcal{B}}}
\newcommand{\defeq}{\ensuremath{=}}
\newcommand{\intd}{\ensuremath{\text{d}}}
\newcommand{\mix}{\ensuremath{\text{mix}}}
\newcommand{\eqdef}{\defeq}
\newcommand{\sign}{\ensuremath{\text{sgn}}}
\newcommand{\erfc}{\ensuremath{\text{erfc}}}
\newcommand{\pmset}{\ensuremath{\{\pm 1\}}}
\newcommand{\KL}{\ensuremath{D_{\text{KL}}}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\inlinenote}[1]{\textcolor{blue}{Note: #1}}
\newcommand{\new}[1]{\textcolor{red}{#1}}

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\parens}{\lparen}{\rparen}
\DeclarePairedDelimiter{\brackets}{[}{]}
\DeclarePairedDelimiter{\ip}{\langle}{\rangle}


\begin{lemma}
  \label{lem:normalized_inner_product}
  Let $(x_1, y_1), \ldots, (x_m, y_m)$ be drawn i.i.d.\ from a $(\thetastar, \sigma)$-corrupted Gaussian model with corruption parameter $p$ and mean norm $\sqrt{d}$.
  Let $h: \R \rightarrow \{0, 1\}$ be a base classifier with accuracy $p > 3/4$, where $p = \E[\I[h(x) = y]]$,
  Let $\vzbar \in \R^d$ be the sample mean vector $\vzbar = \frac{1}{m} \sum_{i=1}^{m} \yhi x_i$, where $\yhi = h(x_i)$.
  Let $\what \in \R^d$ be the unit vector in the direction of $\vzbar$, i.e., $\what = \sfrac{\vzbar}{\norm{\vzbar}_2}$.
  Let $c$ denote the constant in Lemma XX.
  Then we have
  \[
    \prob\brackets*{ \ip{\what, \vmu} \, \leq \, \frac{(4p - 1) \sqrt{dm} + \sqrt{d + 2m \sigma^2 \log 2}}{(1 + c)\sqrt{m} + 2\sigma} } \; \leq \; small \; .
  \]
\end{lemma}
\begin{proof}
    By [Hussein Lemma 3], we have
\[
    \prob\brackets*{ \ip{\norm{\vzbar}_2, \thetastar } \geq  } \geq 1 - (0.95)^{mp} + \delta
\]
\end{proof}










\section{UAT Sketch}

\newcommand{\model}{f_{\theta}}
\newcommand{\modelloss}{\ell_{\theta}}
\newcommand{\advsup}{\sup_{x' \in N_{\epsilon}(x')}}

\note{JU: Including previous notes for reference}
\subsection{Motivation}

The merits of our proposed approach rely on a critical assumption.

\begin{assumption}
    For many classification problems, unlabeled examples are dramatically cheaper to acquire than labeled examples.
\end{assumption}

For example, for large-scale image classification problems, unlabeled examples can be acquired by scraping images off the web, whereas gathering labeled examples requires hiring human labellers.

\subsection{Notation}
A model parameterized by $\theta$ defines a mapping $f_{\theta}: \mathcal{X} \rightarrow \mathcal{Y}$, 
where $\mathcal{X}$ is the input space and $\mathcal{Y}$ is a set of discrete classes. 
Throughout, we take $\ell(\cdot, \cdot)$ to be the $0-1$ loss, and for brevity, use $\ell_\theta(x, y)$ to denote $\mathbbm{1}[\model(x) \neq y]$. 
We define the neighborhood around $x$ as $N_{\epsilon}(x) = \{ x' : \norm{x' - x} \leq \epsilon \}$. 
The adversarial loss at a point $(x, y)$ is then $\advsup \modelloss(x', y)$, 
and the expected adversarial loss is $\mathbb{E}_{(x, y) \sim p}[\advsup \modelloss(x', y)]$, where $p$ is the unknown data distribution.

\subsection{Theoretical Results}
\begin{obs} For all $x, y, \theta$, the adversarial loss is bounded by the natural loss and the unsupervised adversarial loss.
    $$\advsup \modelloss(x', y) \leq \modelloss(x, y) + \advsup \modelloss(x', y')$$
\end{obs}

This is apparent by casework, as when $y' = y$, the LHS and RHS are equivalent, and when $y' \neq y$, then the natural loss is $1$. The main point here is that while the first term, the natural loss, depends on the true label $y$, the unsupervised adversarial loss has no dependence on $y$. This suggests that adversarial generalization may be improved by minimizing an empirical estimate of this upper bound using unlabeled data.

    


			



			






